State estimation in minimal turbulent channel flow: A comparative study of 4DVar and PINN

The state of turbulent, minimal-channel flow is estimated from spatio-temporal sparse observations of the velocity, using both a physics-informed neural network (PINN) and adjoint-variational data assimilation (4DVar). The performance of PINN is assessed against the benchmark results from 4DVar. The PINN is efficient to implement, takes advantage of automatic differentiation to evaluate the governing equations, and does not require the development of an adjoint model. In addition, the flow evolution is expressed in terms of the network parameters which have a far smaller dimension than the predicted trajectory in state space or even just the initial condition of the flow. Provided adequate observations, network architecture and training, the PINN can yield satisfactory estimates of the the flow field, both for the missing velocity data and the entirely unobserved pressure field. However, accuracy depends on the network architecture, and the dependence is not known a priori. In comparison to 4DVar estimation which becomes progressively more accurate over the observation horizon, the PINN predictions are generally less accurate and maintain the same level of errors throughout the assimilation time window. Another notable distinction is the capacity to accurately forecast the flow evolution: while the 4DVar prediction depart from the true flow state gradually and according to the Lyapunov exponent, the PINN is entirely inaccurate immediately beyond the training time horizon unless re-trained. Most importantly, while 4DVar satisfies the discrete form of the governing equations point-wise to machine precision, in PINN the equations are only satisfied in an $L^2$ sense.

==> Letter_to_editor <==
%==========================================
%       Letter:  Revised submission
%==========================================

Dear Prof. Klewicki,

Attached please find our revised manuscript and responses to the reports by the Referees.  Both referee 1 and referee 2 acknowledged the merits of our study and its contributions. They described the manuscript as ``well-written'' and noted that our work is ``worthy of publication''. They also provided some comments that we addressed fully in our responses and in the revisions to the manuscript. 

Referee 1 requested a further comparison of 4DVar and PINNs. In response, we added the following materials:
- Detailed computational cost of both methods in \S3.1.
- Forecasts beyond the assimilation window by marching the terminal PINN-estimated fields using direct numerical simulations.
- New data assimilation tests at a higher Reynolds number, Re_{\tau} = 392, using both 4DVar and PINN.
We hope that our earnest efforts will be recognized by this referee.  

We thank you for your further consideration of our manuscript, and hope that it will be accepted in its revised form for publication in the International Journal of Heat and Fluid Flow. 

Regards
Tamer



%==========================================
%       Letter:  Initial submission
%==========================================
Dear Prof Pollard

Attached please find our manuscript titled “State estimation in minimal turbulent channel flow: A comparative study of 4DVar and PINN”.  We appreciate your consideration of our manuscript for publication in the special issue on machine learning. 

The work compared the benchmark adjoint approach to physics-informed neural networks, for assimilation of experimental data in computational methods.  Some suggested referees are below, with expertise in both fields: 

	Grauer, Samuel <sgrauer@psu.edu>; 
	Koji Fukagata <fukagata@mech.keio.ac.jp>; 
	Yosuke Hasegawa <ysk@iis.u-tokyo.ac.jp>; 
	Vincent Mons <vcnt.mons@gmail.com>; 
	Karthik Duraisamy <kdur@umich.edu>;


Sincerely
Tamer Zaki


